Semi-parametric Network Structure Discovery Models

We propose a network structure discovery model for continuous observations that generalizes linear causal models by incorporating a Gaussian process (GP) prior on a network-independent component, and random sparsity and weight matrices as the network-dependent parameters. This approach provides flexible modeling of network-independent trends in the observations as well as uncertainty quantification around the discovered network structure. We establish a connection between our model and multi-task GPs and develop an efficient stochastic variational inference algorithm for it. Furthermore, we formally show that our approach is numerically stable and in fact numerically easy to carry out almost everywhere on the support of the random variables involved. Finally, we evaluate our model on three applications, showing that it outperforms previous approaches. We provide a qualitative and quantitative analysis of the structures discovered for domains such as the study of the full genome regulation of the yeast Saccharomyces cerevisiae.

==> abstract_gplatnet.tex <==
\begin{abstract}
We propose a network structure discovery model for continuous observations that generalizes linear causal models by incorporating a Gaussian process (GP) prior on a network-independent component, and random sparsity and weight matrices as the network-dependent parameters. This approach provides flexible modeling of network-independent trends in the observations as well as uncertainty quantification around the discovered network structure. We establish a connection between our model and multi-task GPs and develop an efficient stochastic variational inference algorithm for it. Furthermore, we formally show that our approach is numerically stable and in fact numerically easy to carry out almost everywhere on the support of the random variables involved. Finally, we evaluate our model on three applications, showing that it outperforms previous approaches. We provide a qualitative and quantitative analysis of the structures discovered for domains such as the study of the full genome regulation of the yeast \textit{Saccharomyces cerevisiae}.   
% OLD ABSTRACT 
%Given continuous-valued observations from nodes of a network over time, we propose a model and a variational inference algorithm for discovering the structure of the network. The model is built upon linear causal models and we extend them in two directions: (i) we introduce a new latent function with a Gaussian Process prior into the framework in order to model network-independent trends in the observations from nodes, (ii) we represent the structure of the network using random sparsity and weight matrices in a Bayesian framework, and develop an efficient variational method for inference over the network structure. Also, the relationship between the efficiency of the algorithm and the network structure is formally validated. The model and the inference algorithm are evaluated based on their performance on (i) synthetic datasets, (ii) in discovering brain functional connectivity, and (iii) in finding the relationship between property prices in different regions of Sydney. The results indicate that when the number of observations is small in comparison to the number of nodes in the network, the proposed method outperforms other models, and in the other conditions it provides comparable performance to other methods.
\end{abstract}


==> conclusion_gplatnet.tex <==
\section{Conclusion}\label{sec-con}

We introduced and analyzed a new framework for network structure discovery based on continuous-valued observations from nodes of the network over time, and the modeling of a network-independent component as a Gaussian Process. Coupled with an efficient variational inference method for calculating the posterior distribution over the network structure, our theory does not just show that the algorithm is computationally efficient, it also shows that the traditional constraints for identifiability in networks are alleviated: the finiteness of the evidence lowerbound (ELBO) is essentially obtained ``for free". What we get however with additional assumptions that parallel the traditional ones is a non-negligible uplift in the easiness of the task, namely that the expected log-likelihood part, the bottleneck of the ELBO, does not in fact suffer numerical instabilities over most of its support. This result also holds for a broader class of posteriors than the ones we use, opening interesting avenues of applications for concrete distributions.

\noteEB{Need to conclude what the most important things we have achieved are: MTL, efficienty, good results}

==> discuss_gplatnet.tex <==
\section{Discussion}\label{sec-dis}

%%


From the theoretical standpoint, the state of the art goes with substantial constraints that can be related to \textit{identifiability}, \textit{i.e.} the fact that the true model exists, is unique and can be properly recovered. Some can more specifically be related to the radius of convergence of a series of type $\approx \sum_{t\geq 0} z^t$, where $t$ symbolizes time and $z$ can be a real, complex or matrix argument \cite{Hyvarinen2013,Linderman2014}. Thus, plus sampling arguments to control all matrix entries \cite{Hyvarinen2013,Linderman2014} yield \textit{e.g.} the constraints in (\ref{laDLCM1}), (\ref{laDLCM2}). We emphasize that all entries need to be bounded, therefore those techniques do not benefit from the concentration of measure that we exploit to obtain Theorem \ref{thEASYM}. The trick of replacing the analysis over all $t$s by one over a window, rather than alleviating the constraint, substitutes it for other constraints that can be equally restrictive, for example the assumption of stationarity of time series that constrain the expectation and variance of the signal \cite{shimizu2006linear}. 

In our case, such constraints do not appear because time is absorbed in a GP. Also, identifiability \textit{per se} is not anymore a problem since the prior is unique and should therefore be identifiable. Yet, to make a connection with other techniques, we identify it with the difficulty of sampling in the model, that is, getting finite (over the whole support) and numerically stable (over large subsets) estimates. The former problem is that of controlling the non-singularity of $\I -\bA \odot \bW$, which is far easier to handle than bounding its spectral radius like in \cite{Linderman2014}. In short, handle the same objects as in usual approaches \cite{Hyvarinen2013,Linderman2014}, but with weaker constraints. Also, we use these approaches for the default fixation of our parameters, with an uninformative prior over $\{A_{ij}\}$ is chosen ($\meana=0.5$), and 
the prior variances of $\{ W_{ij} \}$ are set to $\varw = 2/N$. 
\noteRN{Edwin, Amir, make sure you agree with these or they need to be changed}

\noteEB{This discussion needs to be significantly reduced. One paragraph at most and merge with conclusion.}

==> model_gplatnet_old.tex <==
\section{Model Specification}
We have a network consisting of $N$ nodes, and we have observed outputs $\by_i$ from each node $i$ at time points $\bt_i$. Therefore, we have a data set $\cD$ consisting of $N$ vector observations $\bY = \{ \by_i\}_{i=1}^N$ and their corresponding observation times $\{ \bt_i\}_{i=1}^N$. The output of node $i$ at time $t$ is denoted by $y_i(t)$, and we assume it is generated by a noise-free latent function $f_i$ as follows:
\begin{equation}
\label{eq:likelihood}
y_i(t) = f_i(t) + \epsilony, \quad \epsilony \sim \Normal(0, \varnoise) \text{,}
\end{equation}
where $\varnoise$ is the observation-noise variance. 
 To model latent function $f_i$, we assume that it is generated by two sources: (i) a network-independent component, which is denoted by $z_i(t)$, and (ii) a network dependent component, i.e., a weighted sum of the inputs received from the rest of the network:
\begin{align}
\label{eq:prior-f-1}
f_i(t) &= z_i(t) + \sum_{\substack{j=1\\j \neq i}}^NA_{ij}W_{ij}\left[f_j(t) + \epsilonf\right] \text{, } \\
\label{eq:prior-f-2}
z_i(t) &\sim \GP(\mathbf{0}, \kernelt(t,t';\btheta)) \text{,} \quad \epsilonf \sim \Normal(0, \varf)  \text{.} 
\end{align}   
\noteEB{Need to be consistent with matrix entry notation. In following sections we use boldface.}
In other words, the output of node $i$ is generated by $z_i(t)$ plus the noisy outputs of all the other nodes. Here, matrix $\bA$ is the adjacency matrix, where $A_{ij} \in \{0,1\}$ represents the existence of a connection (arc) from node $j$ to node $i$. Connections between nodes are weighted by matrix $\bW$, where $W_{ij}\in \mathbb{R}$ determines the weight of the connection from node $j$ to node $i$ (we assume $A_{ii}=W_{ii}=0$). We refer to $\bA$ and $\bW$ as network parameters. It is further assumed that output $f_j(t)$ is not received by node $i$ undistorted, but a zero mean Gaussian noise $\epsilonf \sim \Normal(0, \varf)$ adds to the inputs received by a node from other nodes. 
As for the network-independent component, we assume $z_i(t)$ is distributed as a Gaussian process \citep[GP;][]{Rasmussen:2005}  
with covariance function $\kernelt(t,t';\btheta)$ and  hyperparameters $\btheta$. 
The model is therefore a combination of parametric elements ($\bA$ and $\bW$) and non-parametric elements, i.e., $z_i(t)$, and therefore it is a semi-parametric model.
%
%
\subsection{Prior over Network Parameters \label{sec:prior}}
Equation \eqref{eq:likelihood} defines the likelihood of our observations and Equations \eqref{eq:prior-f-1} and
\eqref{eq:prior-f-2} define the prior over the latent functions given the network parameters $\bA, \bW$. As our goal 
is to infer the structure of the network, these parameters are also random variables and their prior is defined as:
\begin{align}
\label{eq:prior-AW-1}
	p(\bA, \bW) = p(\bA) p(\bW) = \prod_{ij} p(A_{ij}) p(W_{ij}) \text{,} \\
\label{eq:prior-AW-2}
	p(A_{ij}) = \Bernoulli(\meana) \text{,} \quad p(W_{ij}) = \Normal(0, \varw) \text{,}
\end{align}
 where $\Bernoulli(\meana)$ denotes a Bernoulli distribution with parameter $\meana$.
  
Let us denote the values of all latent functions $f_i(t)$ at time $t$ with $\bF(t) = [f_1(t),\dots, f_N(t)]$, and similarly $\bz(t) = [z_1(t),\dots, z_N(t)]$. Hence, we can rewrite Equation \eqref{eq:prior-f-1} as:
\begin{equation}	
	\label{eq:Ft}	
	\bF(t)= (\I -\bA \odot \bW)^{-1}(\bz(t) + \bA \odot \bW\bepsilonf),
\end{equation}
where $\odot$ is the Hadamard (element-wise) product. We refer the model in Equation \eqref{eq:Ft} as the \emph{inverse model}. 
Given $\bz(t)$ and $\bepsilonf$, the random variables $f_i(t)$ are well defined if matrix $(\I -\bA \odot \bW)$ is invertible. Indeed, this is a necessary but not sufficient condition, and as argued in \cite{Hyvarinen2013}, the network will be identifiable if the absolute values of all the elements of $\bA \odot \bW$ are less than one, and also the absolute value of the dominant eigenvalue of $\bA \odot \bW$ is less than one.  Hence, we aim to choose priors such that the network is identifiable. According to the so called circular law \cite{Linderman2014}, given the random matrix $\bM$ of dimensions $N\times N$ with i.i.d entries of variance $1/N$ and zero mean, as $N$ tends to infinity, the spectral distribution of $\bM$ converges to the unit disk in the complex plane. In the case that $\bM$ represents prior distribution over $\bA \odot \bW$, the means of the entries of $\bM$ are zero (since the mean of prior distribution over $W_{ij}$s is zero), and the variance of entries will be $\varw \meana^2$. Based on the circular law, the maximum eigenvalue of $\bA \odot \bW$ will asymptotically be $\stdw \sqrt{N \meana}$, which is required to be less than one. To ensure that this condition is met, a uninformative prior over $\{A_{ij}\}$ is chosen ($\meana=0.5$), and 
the prior variances of $\{ W_{ij} \}$ are set to $\varw = 2/N$. 

